Single top quark cross section measurement in the t-channel at the high-luminosity LHC

We study the precision with which the t-channel single top quark production cross section is expected to be measured in future LHC runs at 14 TeV. The single top final state has a lepton and neutrino from the top quark decay plus two jets, one of which is required to be b-tagged. This measurement is done in the context of the Snowmass 2013 study for the low-luminosity 14 TeV and the high-luminosity 14 TeV LHC as well as for high-luminosity 33 TeV LHC.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf

# use dvipdfm on a mac so that the pdf generated on a mac includes all proper fonts.
UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Darwin)
        DVIPDF = dvipdfm
endif

BASENAME = tchan

default: pdf

ps: ${BASENAME}.tex
	latex  -halt-on-error ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvips -j0  ${BASENAME}.dvi -o ${BASENAME}.ps
	@echo "Output written to ${BASENAME}.ps"

pdf: ${BASENAME}.tex
	latex  -halt-on-error ${BASENAME}
	latex  ${BASENAME}
	bibtex    ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	${DVIPDF} ${BASENAME}
	@echo "Output written to ${BASENAME}.pdf"

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


